Inversion-Free Image Editing with Natural Language

Despite recent advances in inversion-based editing, text-guided image manipulation remains challenging for diffusion models. The primary bottlenecks include 1) the time-consuming nature of the inversion process; 2) the struggle to balance consistency with accuracy; 3) the lack of compatibility with efficient consistency sampling methods used in consistency models. To address the above issues, we start by asking ourselves if the inversion process can be eliminated for editing. We show that when the initial sample is known, a special variance schedule reduces the denoising step to the same form as the multi-step consistency sampling. We name this Denoising Diffusion Consistent Model (DDCM), and note that it implies a virtual inversion strategy without explicit inversion in sampling. We further unify the attention control mechanisms in a tuning-free framework for text-guided editing. Combining them, we present inversion-free editing (InfEdit), which allows for consistent and faithful editing for both rigid and non-rigid semantic changes, catering to intricate modifications without compromising on the image's integrity and explicit inversion. Through extensive experiments, InfEdit shows strong performance in various editing tasks and also maintains a seamless workflow (less than 3 seconds on one single A40), demonstrating the potential for real-time applications. Project Page: https://sled-group.github.io/InfEdit/

==> img/compare-di.tex <==
% \begin{figure}[!htp]
%     \centering
%     \vspace*{-0.25cm}
%     \includegraphics[width=1.0\linewidth]{img/source/compare-di-ddcm.pdf}
%     \caption{Ablation: DDCM inversion vs. Direction Inversion}
%     \label{fig::ddcm vs di}
%     \vspace*{-0.25cm}
% \end{figure}
\begin{figure}[!htp]
    \centering
    \vspace*{-0.25cm}
    \includegraphics[width=\linewidth]{img/source/compare-di-ddcm.pdf}
    \caption{DDCM vs DI. DI doesn't follow the edit objective.}
    \label{fig::ddcm vs di}
    \vspace*{-0.25cm}
\end{figure}


==> img/compare-radar1.tex <==
\begin{figure}[!htp]
    \centering
    \vspace*{-0.25cm}
    \includegraphics[width=1.0\linewidth]{img/source/clip-score.pdf}
    \caption{Placeholder}
    \label{fig::clip}
    \vspace*{-0.25cm}
\end{figure}


==> img/compare-radar2.tex <==
\begin{figure}[!htp]
    \centering
    \vspace*{-0.25cm}
    \includegraphics[width=1.0\linewidth]{img/source/consistency.pdf}
    \caption{Placeholder}
    \label{fig::consistency}
    \vspace*{-0.25cm}
\end{figure}


==> table/compare-cycle.tex <==
\begin{table}[htbp]
\small
\centering
\renewcommand\arraystretch{0.8}
\setlength{\tabcolsep}{0.3mm}{
\centering
\begin{threeparttable}
\begin{tabular}{crrr}
\toprule
\textbf{P2P} & \multicolumn{1}{c|}{\textbf{CLIP Score}$\uparrow$} & \multicolumn{1}{c|}{\textbf{Forward time}$\downarrow$} & \multicolumn{1}{c}{\textbf{Steps}$\downarrow$} \\ 
\cmidrule(r){1-1} \cmidrule(r){2-4}
\textbf{CycleD} & 23.68 & 4.55 $\pm$0.02 & 32 \\
\textbf{VI} & 24.89 & 4.50 $\pm$0.01 & 32 \\
\cmidrule(r){1-1} \cmidrule(r){2-4}
\textbf{LCM + VI} & 24.57 & 2.60 $\pm$0.00 & 15 \\
\bottomrule
\end{tabular}
\footnotesize
\end{threeparttable}
\caption{CycleDiffusion has much lower editing ability as measured by CLIP score}
\label{tab:compare-cyclediff}

}

\end{table}


==> table/sub_task_temp.tex <==
\begin{table*}[htbp]
\small
\centering
  \renewcommand\arraystretch{0.8}
\setlength{\tabcolsep}{0.3mm}{
\begin{threeparttable}
\begin{tabular}{c|c|c|cccc|cc}
\toprule
\toprule
\textbf{Method} & \textbf{Structure}          & \multicolumn{4}{c|}{\textbf{Background Preservation}} & \multicolumn{2}{c}{\textbf{CLIP Similariy}} \\ \midrule
\textbf{Editing}            & \textbf{Distance}$_{^{\times 10^3}}$ $\downarrow$ & \textbf{PSNR} $\uparrow$     & \textbf{LPIPS}$_{^{\times 10^3}}$ $\downarrow$  & \textbf{MSE}$_{^{\times 10^4}}$ $\downarrow$     & \textbf{SSIM}$_{^{\times 10^2}}$ $\uparrow$    & \textbf{Whole}  $\uparrow$          & \textbf{Edited}  $\uparrow$       \\ \midrule
 \textbf{P2P}                & 69.43           & 17.87  & 208.80  & 219.88  & 71.14 &  \underline{25.01}        &  \textbf{22.44}          \\
 \textbf{Masactrl}                & 69.43           & 17.87  & 208.80  & 219.88  & 71.14 &  \underline{25.01}        &  \textbf{22.44}      \\
\midrule
 \textbf{Ours}                & 69.43           & 17.87  & 208.80  & 219.88  & 71.14 &  \underline{25.01}        &  \textbf{22.44}      \\
\midrule
\bottomrule
\end{tabular}
\begin{tablenotes}
   \footnotesize
   \item[*] Placeholder
    \end{tablenotes}
    \end{threeparttable}}
    \vspace{-0.2cm}
\caption{placeholder}
        \label{tab:placeholder}
    \vspace{-0.2cm}
\end{table*}
